Connected Components in Linear Work and Near-Optimal Time

Computing the connected components of a graph is a fundamental problem in algorithmic graph theory. A major question in this area is whether we can compute connected components in $o(\log n)$ parallel time. Recent works showed an affirmative answer in the Massively Parallel Computation (MPC) model for a wide class of graphs. Specifically, Behnezhad et al. (FOCS'19) showed that connected components can be computed in $O(\log d + \log \log n)$ rounds in the MPC model. More recently, Liu et al. (SPAA'20) showed that the same result can be achieved in the standard PRAM model but their result incurs $\Theta((m+n) \cdot (\log d + \log \log n))$ work which is sub-optimal. In this paper, we show that for graphs that contain \emph{well-connected} components, we can compute connected components on a PRAM in sub-logarithmic parallel time with \emph{optimal}, i.e., $O(m+n)$ total work. Specifically, our algorithm achieves $O(\log(1/\lambda) + \log \log n)$ parallel time with high probability, where $\lambda$ is the minimum spectral gap of any connected component in the input graph. The algorithm requires no prior knowledge on $\lambda$. Additionally, based on the \textsc{2-Cycle} Conjecture we provide a time lower bound of $\Omega(\log(1/\lambda))$ for solving connected components on a PRAM with $O(m+n)$ total memory when $\lambda \le (1/\log n)^c$, giving conditional optimality to the running time of our algorithm as a parameter of $\lambda$.

==> Algorithms/spanningforest.tex <==

\section{Spanning Forest Algorithms} \label{sec:sf_all}

In this section, we first present a parallel algorithm that computes the spanning forest of any given graph in $O(\log d + \log\log n)$ time (but not in linear work). 
We choose to present the implementation on an ARBITRARY CRCW PRAM. From PRAM, the implementation on an MPC (in the same running time) with $n^{\delta}$ memory per processor is straightforward for any constant $\delta \in (0,1)$, e.g., see \cite{DBLP:conf/focs/Andoni}.
The previous fastest spanning forest algorithm on PRAM and MPC run in $O(\log d \cdot \log\log n)$ time \cite{liu2020connected}.

Based on the $O(\log d + \log\log n)$-time algorithm for spanning forest, we then adopt our techniques for linear-work connectivity algorithms (\S{\ref{sec:stage1}} to \S{\ref{sec:boosting}}) to get a spanning forest algorithm with $O(m + n)$ work and $O(\log(1/\lambda) + \log\log n)$ running time with high probability.


\subsection{An $O(\log d + \log\log n)$-time Spanning Forest Algorithm} \label{subsec:log_d_sf}

\paragraph{Additional notations for spanning forest.}
For each edge $e$ in the current graph, we use $\hat{e}$ to denote the original edge in the input graph that is \emph{altered} to $e$ during the execution of the algorithm. 
Each edge processor is identified by an original edge $\hat{e}$ and stores the corresponding $e$ in its private memory during the execution.
We use a global field $.f$ for each edge $e$. 
To output the spanning forest, for an original graph edge $\hat{e} = (v, w)$, if at the end of the algorithm $\hat{e}.f = 1$, then it denotes that the graph edge $(v, w)$ is in the spanning forest. 
Otherwise if $\hat{e}.f = 0$, then the edge $(v, w)$ is not in the spanning forest computed by the algorithm. 

\begin{framed}
\noindent \textsc{SpanningForest}$(G = (V, E))$:
\begin{enumerate}
    \item Run \textsc{Reduce}$(V, E, 10^6 \log\log n)$ to obtain the current graph $G'$. \label{alg:sf:step1}
    \item For \emph{slice} $j$ from $0$ to $10 \log\log n$:  \label{alg:sf:step2}
    \begin{enumerate}
        \item \textsc{ExpandCutoff}$(j)$. \label{alg:sf:step2a}
        \item \textsc{Vote}$(V(G'))$. \label{alg:sf:step2b}
        \item \textsc{TreeLink}$(j)$. \label{alg:sf:step2c}
        \item \textsc{Shortcut}$(V)$. \label{alg:sf:step2d}
        \item \textsc{Alter}$(E(G'))$. \label{alg:sf:step2e}
    \end{enumerate}
\end{enumerate}
\end{framed}

In Step~\ref{alg:sf:step1} of \textsc{SpanningForest}$(G)$, the algorithm runs \textsc{Reduce}$(V, E, 10^6 \log\log n)$ to reduce the number of vertices in the current graph $G'$ to $n / (\log n)^{1000}$ w.p. $1 - n^{-7}$ (Lemma~\ref{lem:polylog_shrink_reduce}). 
In order to output a spanning forest, we make the following changes to \textsc{Reduce}. 
During the execution of \textsc{Reduce}, whenever a \textsc{Matching}$(E)$ is called, in its Step~\ref{alg:matching:s8}, if $v.p$ is updated to $u$ then write the edge $e \coloneqq (u, v)$ to the private memory of the vertex processor corresponding to $v$ (arbitrary win). 
After Step~\ref{alg:matching:s8} of \textsc{Matching}$(E)$, for each vertex $v$ such that the edge in the private memory of $v$ is updated in Step~\ref{alg:matching:s8}, execute $v.\hat{e}.f = 1$, where $v.e$ is the edge stored in $v$ and $v.\hat{e}$ is the edge in the original input graph corresponding to $v.e$ in the current graph, and $v.\hat{e}.f = 1$ indicates that this original edge is in the output spanning forest. 
For a detailed proof of correctness, see Section 4.1 of \cite{liu2020connected}.

We call each of the $10 \log\log n$ iterations of Step~\ref{alg:sf:step2} of \textsc{SpanningForest}$(G)$ a \emph{slice}. 
Each slice contains $5$ steps. 
We outline the functionality of each step here, then give detailed implementations and proofs for each of it later in this section. 

In Step~\ref{alg:sf:step2a}, 



\Cliff{TBD}TBD

\subsubsection{} \label{subsubsec:}


\begin{framed}
\noindent \textsc{ExpandCutoff}$(j)$:
\begin{enumerate}
    \item Each vertex is either \emph{live} or \emph{dormant} in a step. Mark every vertex as \emph{live} at the beginning.\label{alg:expcut:step1}
    \item For each root: assign a block of size $(\log n)^{100 \cdot 2^j}$. \label{alg:expcut:step2}
    %\item For each graph arc $(v, w)$: if $v$ is live before Step~\ref{alg:expcut:step3} then use $h_V$ to hash $v$ into $H(v)$ and $w$ into $H(v)$, else mark $w$ as \emph{dormant}. \label{alg:expcut:step3}
    \item For each graph arc $(v, w)$: use $h_V$ to hash $v$ into $H(v)$ and $w$ into $H(v)$. \label{alg:expcut:step3}
    \item For each hashing done in Step~\ref{alg:expcut:step3}: if it causes a \emph{collision} (a cell is written by different values) in $H(u)$ then mark $u$ as \emph{dormant}. \label{alg:expcut:step4}
    \item Repeat the following until there is neither live vertex nor hash table getting a new entry:\label{alg:expcut:step5}
        \begin{enumerate}
            \item For each vertex $u$: for each $v$ in $H(u)$: if $v$ is dormant before Step~\ref{alg:expcut:step5a} in this iteration then mark $u$ as \emph{dormant}, for each $w$ in $H(v)$: use $h_V$ to hash $w$ into $H(u)$.  \label{alg:expcut:step5a}
            \item For each hashing done in Step~\ref{alg:expcut:step5a}: if it causes a collision in $H(u)$ then mark $u$ as \emph{dormant}.\label{alg:expcut:step5b}
        \end{enumerate}
\end{enumerate}
\end{framed}
